Scalable Rate Control for Traffic Engineering with Aggregated Flows in Software Defined Networks

To increase the scalability of Software Defined Networks (SDNs), flow aggregation schemes have been proposed to merge multiple mouse flows into an elephant aggregated flow for traffic engineering. In this paper, we first notice that the user bit-rate requirements of mouse flows are no longer guaranteed in the aggregated flow since the flow rate decided by the TCP allocation is usually different from the desired bit-rate of each user. To address the above issue, we present a novel architecture, named Flexible Flow And Rate Management (F$^2$ARM), to control the rates of only a few flows in order to increase the scalability of SDN, while leaving the uncontrolled flows managed by TCP. We formulate a new optimization problem, named Scalable Per-Flow Rate Control for SDN (SPFRCS), which aims to find a minimum subset of flows as controlled flows but ensure that the flow rates of all uncontrolled flows can still satisfy the minimum required rates by TCP. We prove that SPFRCS is NP-hard and design an efficient algorithm, named Joint Flow Selection and Rate Determination (JFSRD). Simulation results based on real networks manifest that JFSRD performs nearly optimally in small-scale networks, and the number of controlled flows can be effectively reduced by 50% in real networks.

==> Algorithm.tex <==
%\makeatletter
%\renewcommand*{\ALG@name}{Algorithm}
%\makeatother

% this is for phase label


\clearpage

\begin{algorithm}[t]
    \caption{Flow Selection (FS)}
    %\label{alg:algo}
    \begin{algorithmic}[1]    
        %\REQUIRE%~\\
        \INPUT
        A network $G=(V,E)$, the capacity $c(e)$ and correlation $\gamma(e)$ of each link $e\in E$, and a set of flows $F$ with the rate demand $d(f)$ and path $p(f)$ for each $f\in F$
            %$G$: ($V$, $E$)\\
            %$F$: The set of request flows in the network\\
            %$\gamma(e)$: The sum of correlated value of flow which go through $e$, $\ForAll e \in E$\\
            %$p(f)$: The routing path of flow $f$, $\ForAll f \in F$\\
            %$d(f)$: The demands of $f$, $\ForAll f \in F$\\
            %$c(e)$: The link capacity of $e$, $\ForAll e \in E$\\
        %\ENSURE%~\\
        \OUTPUT
            The selected configuration $A_s(e)$ of each link $e\in E$%
            %$A_s(e)$ = The selected configuration of $e$ , $\ForAll e \in E$
        %\State \textit{Initial}:
        %\State For each link $e\in E$, $\rho(e)\leftarrow c(e) - \sum_{f: p(f)\ni e} d(f)$;
        %\State \textit{Configuration stage}:
        %\NoNumber{\underline{\textbf{Configuration State}}}
        %\State \underline{\textbf{Configuration State}}
        \phase{Configuration Stage}
        \State $A(e)[f]:=$ The configuration of link $e$ for target flow $f$;
        \ForAll {link $e$ in $E$}
            \ForAll {flow $f:p(f)\ni e$}
                %\State $\rho(e)$ recovery to original
                %
                \State $\rho(e)\leftarrow c(e) - \sum_{f': p(f')\ni e} d(f')$;
                
                \ForAll{flow $f':p(f')\ni e$}
                    \State The rate of $f'$ in $A(e)[f]\leftarrow d(f')$;
                \EndFor
                %\State Sort the flows on link $e$ in ascending order by $d(f)$;
                \ForAll {$f'$ on link $e$ with the largest $d(f') < d(f)$}
                    \If {$\rho(e) - (d(f) - d(f')) > 0$}
                        \State The rate of $f'$ in $A(e)[f]$ $\leftarrow$ $d(f)$; 
                        \State $\rho(e) \leftarrow \rho(e) - (d(f) - d(f'))$;
                    \EndIf
                \EndFor
            \EndFor
            %\State $A(e)$ = The configurations have largest number of flows with the same rate 
        \EndFor
        \phase{Selection Stage}
        %\State \textit{Selection stage}:
        \State The set of controlled flows $\mathbb{C} \leftarrow \emptyset$;
        \ForAll {link $e \in E$ with the highest $\gamma(e)$ }
            \ForAll {configuration $n \in A(e)$}
                %\State Initial: $\pi_{e}(n) = 0$
                \State The profit $\pi_{e}(n) \leftarrow 0$;
                %\State $value(f)\leftarrow 0, \ForAll f \in F^{c}_{e}(n)$ : whether the $f \in F^{c}_{e'}(n')$
                %\ForAll {$f\in F$}%F_{e}^{c}(n)$}
                %\State $value(f):= $ whether $f\in F_{e'}^{c}(n')$ where $e'\neq e$;
                %\State $value(f)\leftarrow 0$;
                %\EndFor
                \ForAll {link $e' \in E, e' \neq e$}
                    \ForAll {configuration $n' \in A(e')$}
                        \State $value(n')\leftarrow 0$;
                        \ForAll {flow $f \in F^{c}_{e'}(n') \setminus \mathbb{C}$}
                            \If {$f \in F^{c}_{e}(n) \setminus \mathbb{C}$}
                                %\State $value(f) = 1$
                                \State $value(n') \leftarrow value(n') + 1$;
                            \EndIf
                        \EndFor
                    \EndFor
                    \State $\pi_e(n) \leftarrow \pi_e(n) + \displaystyle\max_{n'\in A(e')}\{value(n')\}$;
                \EndFor
                %\ForAll {$f \in F^{c}_{e}(n) \setminus \mathbb{C}$}
                %    \State $\pi_{e}(n) = \pi_{e}(n) + value(f)$
                %\EndFor
                \State $\pi_{e}(n) \leftarrow \frac{\pi_{e}(n)}{|F^{c}_{e}(n) \setminus \mathbb{C}|}$;
            \EndFor
            \State $A_s(e)\leftarrow$ configuration $n$ with $\displaystyle\max_{n\in A(e)}\pi_{e}(n)$;
            \State $\mathbb{C} \leftarrow \mathbb{C} \cup F^{c}_{e}(A_s(e))$;
        \EndFor\\
        \Return $A_s$;%\\
    \end{algorithmic}
\end{algorithm}
%The controlled flow set which is selected from FS phase
\begin{algorithm}[t]
    \caption{Rate Determination (RD)}
    %\label{alg:algo}
    \begin{algorithmic}[1]    
        \INPUT%~\\
            A network $G=(V,E)$, the capacity $c(e)$, correlation $\gamma(e)$, and selected configuration $A_s(e)$ of each link $e\in E$, and a set of flows $F$ with the rate demand $d(f)$, path $p(f)$, and priority $w(f)$ for each $f\in F$%
            %$G$ = ($V$, $E$)\\
            %$F$ = The flow on the network\\
            %$\gamma(e)$ = The sum of correlated value of flows which go through $e$, $\forall e \in E$\\
            %$p(f)$ = The routing path of $f$, $\forall f \in F$\\
            %$d(f)$ = The demands of $f$, $\forall f \in F$\\
            %$w(f)$ = The priority of $f$, $\forall f \in F$\\
            %$\rho(e)$ = The residual bandwidth of $e$, $\forall e \in E$\\
            %$A_s$ = The result from \textit{FS phase}
        \OUTPUT%~\\
            The set of controlled flows $\mathbb{C}$%
        \phase{Initialization begin}
        \ForAll{$n \in A_s$}
            \State $\mathbb{C} \leftarrow \mathbb{C} \cup F^{c}_{e}(n)$;
        \EndFor
%        \State Run \textit{TCP allocation} procedure;
        \ForAll {$e \in E$}
            \State $\rho(e) \leftarrow c(e)$;
            \ForAll {$f\in F^c_e(A_s(e))$}
                \State $r_f\leftarrow d(f)$;
%                \ForAll {$e'\in p(f)$}
                \State $\rho(e) \leftarrow \rho(e) - r_f$;
%                \EndFor
            \EndFor
            \ForAll {$f\in F(e)\setminus F^c_e(A_s(e))$}
                \State $r_f\leftarrow$ target rate of $A_s(e)$;
                \State $\rho(e) \leftarrow \rho(e) - r_f$;
            \EndFor
        \EndFor
        \phase{Initialization end}
        \ForAll {$e \in E$ with the highest $\gamma(e)$ } 
            \State $TC \leftarrow F(e)\cap(\mathbb{C}\setminus F^{c}_{e}(A(e)))$;
            \State $g\leftarrow \infty$;
%            \ForAll{$f\in F_e^c(A(e))$}
%            \EndFor
            %\State $Allocate(f) = \rho(e) * \frac{w(f)}{\sum_{f \in F^{c}_{e}(A(e))} w(f)}$
%            \ForAll {$f \in F^{c}_{e}(A(e))$}
%                \State $Allocate(f) = \rho(e) * \frac{w(f)}{\sum_{f \in F^{c}_{e}(A(e))} w(f)}$;
%            \EndFor
            \Repeat
                \ForAll {$e' \in \displaystyle\bigcup_{f\in F^c_e(A(e))} p(f)\setminus \{e|\rho(e)=0\}$}
                \State $g(e') \leftarrow 0$;
%                    \State $\rho_p(e)$ = The $\rho(e)$ proportionally allocated to the $f$ go through $e$
                    \ForAll {$f \in F^{c}_{e}(A(e))\setminus TC \wedge  \displaystyle\min_{e\in p(f)}\rho(e)>0$}
                        \If{$f\in F^{c}_{e'}(A(e'))$}
                            \State $g(e') \leftarrow g(e')+w(f)$;
                        \EndIf
                    \EndFor
                    \State $g(e')\leftarrow \frac{\rho(e')}{g(e')}$;
                    \If{$g(e') < g$}
                        \State $g \leftarrow g(e')$;
                    \EndIf
                \EndFor
                \ForAll {$f \in F^{c}_{e}(A(e))\setminus TC \wedge  \displaystyle\min_{e\in p(f)}\rho(e)>0$}
                    \State $r_f\leftarrow r_f+ g\cdot w(f)$;
                    \ForAll {$e\in p(f)$}
                        \State $\rho(e) \leftarrow \rho(e) - g\cdot w(f)$;
                    \EndFor
                    %\State $r_f = d(f) + min(Allocate(f) , min(\rho_p(e) | e \in p(f)))$
%                    \State $r_f \leftarrow r_f $;
                    %\State $\rho(e) = \rho(e) - min(Allocate(f) , min(\rho_p(e) | e \in p(f)))$
                \EndFor
            \Until{($\rho(e)=0) \vee (\forall f \in F^{c}_{e}(A(e)), \displaystyle\min_{e \in p(f)}\rho(e)=0)$}
            \State Run \textit{TCP allocation} procedure with input $(G, c, F, p, r, \mathbb{C}\setminus TC)$;
            %\State Check whether the allocation can satisfy all the flow demands
            \If{the allocation can satisfy all the flow demands}
                \State $\mathbb{C} \leftarrow \mathbb{C} \setminus TC$;
                %\State Update $\rho(e), \forall e \in E$ with $r_f$ where $f \in F^{c}_{e}(A(e)$
            \Else
                \State Recover all $r_f$ and $\rho(e)$ to the previous status;
            \EndIf
        \EndFor\\
        \Return $\mathbb{C}$;
    \end{algorithmic}
\end{algorithm}
%\makeatletter
%\renewcommand*{\ALG@name}{Procedure}
%\renewcommand{\thealgorithm}{}
%\makeatother

\makeatletter
\newcounter{procedure}
\newfloat{procedure}{htbp}{loa}[procedure]
\floatname{procedure}{Procedure}
\renewcommand{\theprocedure}{\arabic{procedure}}
\makeatother


\begin{procedure}[t]
    \caption{TCP Allocation}
    %\label{alg:algo}
    \begin{algorithmic}[1]
        \INPUT%~\\
        A network $G=(V,E)$, the capacity $c(e)$ for each link $e\in E$, a set of flows $F$ with path $p(f)$ for each $f\in F$, and the allocated rate $r_f$ of each controlled flow $f\in \mathbb{C}$%, and a set of temporarily controlled flows $TC$%        
            %$F$ = The flow on the network\\
            %$p(f)$ = The routing path of $f$, $\forall f \in F$\\
            %$\rho(e)$ = The residual bandwidth of $e$, $\forall e \in E$\\
            %$TC$ = The set of temporarily uncontrolled flows
        \OUTPUT%~\\
            %$R(f)$ = the rate of each uncontrolled flow
            The rate $r_f$ of each uncontrolled flow $f$%
        %\State Initial: 
        \phase{Initialization begin}
        \State $E'\leftarrow E$;
        \State $c'(e) \leftarrow c(e)-\displaystyle\sum_{f\in F(e) \cap \mathbb{C}} r_f, \forall e \in E$;
        \State $F' \leftarrow F \setminus \mathbb{C}$; %\setminus TC)$;
        \State $F'(e)\leftarrow F(e)\cap F'$;
        \State $r_f \leftarrow 0, \forall f \in F'$;
        \phase{Initialization end}
        %\State $R(f)$ = 0, $\forall f \in F$ 
        %\State
        \Repeat
            %\ForAll{$e \in E'$}
            %    \State Share the $\rho(e)$ to each $f$ goes through $e$
            %\EndFor
            %\ForAll{$f \in F'$}
            %    \State $Add(f)$ = min(the resource from the $e | \forall e \in p(f)$) 
            %    \State $R(f)$ = $R(f) + Add(f)$
            %\EndFor
            
            % time complexity???? the same? |E|^2|F|
            \ForAll{$f \in F'$}
                \State $bw(f) \leftarrow \displaystyle\min_{e\in p(f)} \{ \frac{c'(e)}{|F'(e)|} \}$;%, \forall f\in F'$;
                %\State $r_f = r_f + Add(f)$;
            \EndFor 
            \ForAll{$e \in E'$}
                \If{$c'(e) = \sum_{f\in F'(e)} bw(f)$}
                    \State $r_f \leftarrow bw(f),\forall f\in F'(e)$;
                    \State $E' \leftarrow E' \setminus \{e\}$;
                    \State $F' \leftarrow F' \setminus F'(e)$;
                \EndIf
            \EndFor
            \ForAll{$e \in E'$}
                \State $c'(e) \leftarrow c'(e) - \sum_{f\in F'(e)} r_f$;
                \State $F'(e)\leftarrow F'(e)\cap F'$;
            \EndFor
        \Until{$E' = \emptyset \wedge F' = \emptyset$}\\
        \Return $r_f, \forall f\in F$; %$R(f)$;
    \end{algorithmic}
\end{procedure}

==> Discussion.tex <==
\section{Discussion}
%In this section, we discuss how to implement the JFSRD in the state-of-art SDN architecture.

%\emph{How do we know the information of service level for each flow?}\\
%In this paper,
{\color{black} 
%\subsection{Flow Classification}
%First of all, in this paper, we assume that all the rate demands of different user applications are given in the network. However, in practice, the service levels of flows may not be well-defined in advance. In such cases, the SDN controller can be equipped with a flow classifier (e.g., FlowQoS \cite{FlowQoS}) to classify the flows into different service levels based on their application types. Generally speaking, flow classifier is used to categorize network traffic according to various parameters (e.g., source IP address, destination IP address, protocol, source port, and destination port) into a number of traffic classes so as to provide different service levels for the flows according to their traffic classes. Note that although the requirement of packet inspection for flow classification is inevitable, the system does not postpone the routing service of any newly added flow since the flow can be forwarded with a default policy before it is classified. In the following, we describe how to implement F$^2$ARM and JFSRD in the state-of-art SDN architecture.




\subsection{Dynamic Case}
In real networks, flows may join or leave dynamically and flow demand rates may increase or decrease.
Since re-computing a solution for any change is computation-intensive, the system tends to locally update the solution to adapt to the changes. 
To deal with the more realistic scenarios, the system applies the two phases of JFSRD depending on different conditions as follows.
%In addition, each rate demand may vary during the transmission.  
%Our approach can also adapt well to the dynamic environment as follows. 
Generally speaking, it suffices to control the unsatisfied flows after the dynamic changes.
More specifically, as the flows vary in the network over time, the system does nothing until a flow demand cannot be satisfied.
In such cases, the system executes JFSRD for the first time.
Subsequently, when a rate demand increases, if the flow is still satisfied by the original rate allocation, the system does nothing.
Otherwise, the system will set it to be controlled temporarily, trace back the state of other flows, and re-execute the RD phase. 
%and re-executes the RD phase.
When a rate demand decreases, the system does nothing because the flow is still satisfied by the same configuration.
When a flow leaves, the system will check whether any flow becomes unsatisfied.
If so, %there must be some flow whose rate was originally bounded by the leaving flow while unbounded now so that it uses the allocated rates of other flows.
%Thus, 
the system %only needs to 
sets the these flows to be controlled temporarily,
%that visit the links on the routing path of the leaving flow to be controlled temporarily,
and then re-executes the RD phase.
%Hence, the system only need to re-execute the RD phase in some links which the leaving flow goes through.
When a flow joins, JFSRD will set it to be controlled temporarily, trace back the state of other flows, and re-execute the RD phase. 
%to all of the link since this situation is similar to that when a rate demand increases.
The local update mechanism may increase the gap between the current solution and the optimal solution. Hence, the system periodically computes JFSRD to rearrange the flow statuses so as to minimize the number of controlled flows.
}

%In addition, when the controlled flow have increased to more than the 60 percent of the total number of flows JFSRD will also be re-triggered.


%http://flowgrammable.org/sdn/openflow/message-layer/queue-1/#tab_ofp_1_2

%In this paper, we assume that all the rate demands of different user applications are given in the network. Otherwise, in the system, the SDN controller can classify the flows into different service levels based on their application types (e.g., FlowQoS \cite{FlowQoS}).  Based on the rate demands, JFSRD facilitates the SDN controller to find a subset of controlled flows and to calculate the proper rates of these flows.  Subsequently, the SDN controller employs SDTCP \cite{SDTCP} mechanism at the network side, which extends OpenFlow \cite{OpenFlowSwitch} to adjust the TCP window size to accurately control the rate of flow. More specifically, the SDN controller based on the result installs flow entries with MOD\_WINDOW action on the OpenFlow switches which are on the paths of the corresponding flows. In addition, since TCP is an end-to-end protocol and the sender adjusts the flow rate according to the TCP window size of the ACK packet from the receiver, therefore the flow entry only needs to be installed on \emph{one} switch on the path from the receiver to the sender so as to modify the TCP window size of the ACK packet. On the other hand, similarly, the per-flow control mechanism can also be implemented by modifying the field of window size in the packet header via the middlebox \cite{Middlebox}.

%\subsection{TCAM Utilization}
%To achieve the per-flow control, the SDN controller installs the flow entry on one switch on the path of each controlled flow. However, since the number of TCAM entries on each switch is limited, it is necessary to consider the suitable switch to install the flow entry for each controlled flow. It is similar to match each flow to a TCAM entry on a switch. Therefore, the problem can be reduced to the \textit{maximum bipartite matching} problem, which aims to find the maximum matching in the given bipartite graph, and solved by Hungarian algorithm \cite{Hungarian}. More specifically, each controlled flow and each TCAM entry can be regarded as a node in the left and the right partites, respectively. Afterward, each node in the left partite has an incident edge with the node in the right partite iff the flow entry of the corresponding controlled flow can be installed on the corresponding the TCAM entry of the switch. Since the number of flows is $|F|$, the maximum number of the nodes constructed in the right partite corresponding to the TCAM entries of each switch can be bounded at $|F|$. Thus, the complexity of the transformation is $O(|V||F|^2)$, which is clearly in polynomial time.

    

%\subsection{Dynamic Adaptive Mechanism}
%The flows may join or leave dynamically in the real network. In addition, each rate demand may vary during the transmission. Since re-computing a solution for any change is compute-intensive, it is suggested to locally update the solution to adapt to the small changes. 
%Our approach can also adapt well to the dynamic environment as follows. Generally speaking, it suffices to control these unsatisfied flows after the dynamic changes. More specifically, JFSRD does not react %real-timely
%to the decreasing rate demands since these flows are still satisfied after the changes.

%\textcolor{red}{
%When a rate demand increases, the flow may also be satisfied by the rate allocation of JFSRD thus we do not need to change anything in this situation. When the flow becomes unsatisfied, no matter it status is controlled or uncontrolled sets it to controlled. After that, recovery all flow rates to the demand and re-execute the RD phase. When a flow leaves, JFSRD will run TCP procedure and check whether any flow becomes unsatisfied. In this case, the reason of unsatisfied flow is that some bounded flow have been released by the leaving flow. So we only need to re-execute the RD phase in some links which the leaving flow goes through. When a flow joins, JFSRD will set it to controlled and re-execute the RD phase to all of link. Because this situation is similar to flow rate demand increases.
%}
%first we will check the flow state (i.e. controlled or uncontrolled). If it is controlled, we may base on its rate demand increase the bandwidth of allocation. After that, we will execute RD phase again.


%When a flow leaves, 1) if it is controlled, ... 2) if it is not, ....

%When a flow joins,


%The local update mechanism may increase the gap between the current solution and the optimal solution. Thus, the SDN controller can periodically employ JFSRD to rearrange the flow statuses so as to minimize the number of controlled flows.
